Dynamic Qubit Routing with CNOT Circuit Synthesis for Quantum Compilation

Many quantum computers have constraints regarding which two-qubit operations are locally allowed. To run a quantum circuit under those constraints, qubits need to be mapped to different quantum registers, and multi-qubit gates need to be routed accordingly. Recent developments have shown that compiling strategies based on the Steiner tree provide a competitive tool to route CNOTs. However, these algorithms require the qubit map to be decided before routing. Moreover, the qubit map is fixed throughout the computation, i.e. the logical qubit will not be moved to a different physical qubit register. This is inefficient with respect to the CNOT count of the resulting circuit. In this paper, we propose the algorithm PermRowCol for routing CNOTs in a quantum circuit. It dynamically remaps logical qubits during the computation, and thus results in fewer output CNOTs than the algorithms Steiner-Gauss and RowCol. Here we focus on circuits over CNOT only, but this method could be generalized to a routing and mapping strategy on Clifford+T circuits by slicing the quantum circuit into subcircuits composed of CNOTs and single-qubit gates. Additionally, PermRowCol can be used in place of Steiner-Gauss in the synthesis of phase polynomials as well as the extraction of quantum circuits from ZX diagrams.

==> eptcsdata.tex <==
\providecommand{\firstpage}{363}
\providecommand{\publicationstatus}{S. Gogioso, M. Hoban (Eds.):\\
Quantum Physics and Logic (QPL) 2022\\
EPTCS 394, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.394.18}{10.4204/EPTCS.394.18}}
\pdfoutput=1

